Prospects for Simulating a Qudit Based Model of (1+1)d Scalar QED

We present a gauge invariant digitization of $(1+1)$d scalar quantum electrodynamics for an arbitrary spin truncation for qudit-based quantum computers. We provide a construction of the Trotter operator in terms of a universal qudit-gate set. The cost savings of using a qutrit based spin-1 encoding versus a qubit encoding are illustrated. We show that a simple initial state could be simulated on current qutrit based hardware using noisy simulations for two different native gate set.

==> TrotterOperator.tex <==

As previously mentioned the time evolution operator $e^{-i t \hat{H}}$ has systematic error $\mathcal{O}(t \delta t)$ where $\delta t$ is the Trotter step size. While work has shown that large trotter step sizes are capable of carrying out faithful evolution \cite{Gustafson_2019,gustafson2019benchmarking} for the Transverse Ising model. It is important to examine fidelity of the Trotter operator for the system we are interested in. The fidelity is defined as
\begin{equation}
    \label{eq:fidelity}
    \mathcal{F} = |\langle \psi_i|U_{exact}^{\dagger}(\delta t) U_{trot}(\delta t)|\psi_i\rangle|^2.
\end{equation}
In Fig. \ref{fig:trotter_fidelity} we show the fidelity of Trotter operator acting on the state,
\begin{equation}
\label{eq:initial_state}
    |\psi_i\rangle = \frac{1}{\mathcal{N}} \hat{U}^+_1 |gs\rangle,
\end{equation}
which approximately corresponds the creation of $\phi^{\dagger} \phi$ state across site 1. While there are some resurgences at larger $\delta t$ for the lower spin truncations these are not significant enough to warrant using a larger Trotter step. The likely reason for this this quantum state is heavily entangled and preserving this entanglement requires a smaller Trotter steps using the traditional bound of $\delta t < 1$. 

\begin{figure}[!th]
    \centering
    \includegraphics[width=0.5\textwidth]{fidelitiesvsU.pdf}
    \caption{Fidelity of Trotter operator as a function of U and $\delta t$ for four different spin Truncations with $X=2$ and $Y=1$ and 4 sites.}
    \label{fig:trotter_fidelity}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{SpectrumU4Y1X2.pdf}
    \caption{Energy spectrum for low lying energy states corresponding to approximate single meson states as a function of spin truncation for $U=4.0$, $Y=1.0$, and $X=2.0$.}
    \label{fig:spectrum}
\end{figure}
Up until now the discussion has largely focused on qudit based architectures. However for implementation on near term devices it is best to focus on the spin-1 truncation but the methods are generalizable. The model parameters are set to $U=4.0$, $Y=1.0$, and $X=2.0$. This is done so that a spin-1 truncation is relatively accurate and dynamics are accessible for few Trotter steps. The spectrum for the low lying energy states for spin truncation upto $s_{max} = 6$ is shown in Fig. \ref{fig:spectrum}. We can see that there is a small discrepancy between the spin-1 and spin-2 truncations that correspond to at most 6 to 7 per-cent. However the discrepancies between spin 2 and higher truncations is negligible. This indicates that while there is some systematic error between the original theory and this spin 1 truncation is acceptable for initial testing of qutrit based architectures.

==> ancillary.tex <==
\subsection{Observables}
Key observables in quantum field theories are correlators of which two point correlators (propogators) are the most simple. For our model we can write this correlator as
\begin{equation}
    \label{eq:twopointcorrelator}
    C(x - y, t) = \langle \Omega | e^{i t \hat{H}} \hat{U}^{-}_x e^{-i t \hat{H}} \hat{U}^{+}_y |\Omega\rangle,
\end{equation}
where $|\Omega\rangle$ is the groundstate of $\hat{H}$ and $\hat{U}^{\pm}_x$ is a source/sink operator for the ``meson" at the site $x$ and raise or lower the spin on a state by one. For the spin-1 truncation the matrix for these operators are,
\begin{equation}
    \label{eq:sourcesink}
    \hat{U}^+ =
    \begin{pmatrix}
    0 & 1 & 0 \\
    0 & 0 & 1 \\
    0 & 0 & 0 \\
    \end{pmatrix} \text{ and }
    \hat{U}^- = 
    \begin{pmatrix}
    0 & 0 & 0 \\
    1 & 0 & 0 \\
    0 & 1 & 0 \\
    \end{pmatrix}.
\end{equation}
While preparing the ground state of the model is not trivial using Monte carlo methods (cite Hank, cite Hank and Erik) it is possible to sample from the approximate ground state using the density matrix $\hat{\rho} = e^{-\beta \hat{H}}$. We can then measure this by calculating,
\begin{equation}
    \label{eq:correlatorRho}
    C(x - y, t) \approx \frac{Tr(e^{-i t \hat{H}} \hat{U}^+_x \hat{\rho} e^{i t \hat{H}} \hat{U}^-_y)}{ Tr(\hat{\rho} \hat{U}^-_y \hat{U}^+_x)}.
\end{equation}
Sampling this is relatively straight forward. We can use Monte Carlo methods to generate configurations that sample from the ends of the density matrix $|\psi_i\rangle\langle \psi_j| =  \hat{\rho}_{i, j}$. Up to an overall normalization we can write this quantity as
\begin{equation}
    \label{eq:quantumstatepropogator}
    C(x - y, t) \approx \sum_{i, j} \langle \psi_j | e^{i t \hat{H}} U^{-}_y e^{-i t \hat{H}} U^{+}_x |\psi_i\rangle.
\end{equation}
At first glance the inclusion of the operators $U^{\pm}_x$ is problematic because they are neither hermitian nor unitary, however this will not be a problem as we can write these as a linear combination of operators that are hermitian and unitary. Explicitly this decomposition can be written as follows, 
\begin{equation}
    \label{eq:sourcesinkdecomp}
    \begin{split}
    \hat{U}^+ &= (\hat{X}^{0, 1}\hat{X}^{1, 2} + \hat{X}^{0, 1}\hat{Z}^{2}\hat{X}^{1, 2}) / 2\\
    \text{and}& \\
    \hat{U}^- &= (\hat{X}^{1, 2}\hat{X}^{0, 1} + \hat{X}^{1, 2}\hat{Z}^{2}\hat{X}^{0, 1}) / 2.
    \end{split}
\end{equation}
In order to measure these correlators we need to cleverly map our problem onto a modified version of (Cite Lamm, Yukari, Scott). Suppose we have two operators $\hat{W}_i$ and $\hat{V}^j$ that take the qutrits from the initial computational state to the states  $\hat{U}^+_y|\psi_i\rangle$ and $|\psi_j\rangle$ respectively. It should be noted that these will be relatively simple operators to construct. Next we will need one ancilla qubit\footnote{This can easily mapped onto a subspace of a qutrit as well. A qubit is used for simplicity's sake.} that will be prepared in the state $|+\rangle = (|0\rangle + |1\rangle)/2$. Then given controlled versions of the operators $\hat{W}_i$ and $\hat{V}_j$ we can create an initial superposition of states,
\begin{equation*}
    |\Psi'\rangle = (|0\rangle|\psi_j\rangle + |1\rangle\hat{U}^+_x|\psi_i\rangle)/2.
\end{equation*}
The next step involves applying time time evolution operator $e^{-i t \hat{H}}$ on the working qutrits which gives us the state,
\begin{equation}
\label{eq:timeevolved}
\begin{split}
    |\Psi''\rangle = & \Big(|0\rangle e^{-it\hat{H}}|\psi_j\rangle\\
    &+ |1\rangle e^{-it\hat{H}}\hat{U}^+_x|\psi_i\rangle\Big)/2.
    \end{split}
\end{equation}
Now if apply a controlled $\hat{X}^{1, 2}\hat{X}^{0, 1}$ is applied to the state in Eq. (\ref{eq:timeevolved}) we get the state
\begin{equation}
    \label{eq:timeevolvedxx}
    \begin{split}
        |\Psi''_{xx}(y)\rangle &= \Big(
    |1\rangle \hat{X}^{1, 2}_y \hat{X}^{0, 1}_y e^{-it\hat{H}}\hat{U}^+_x|\psi_i\rangle\\
    &+|0\rangle e^{-it\hat{H}}|\psi_j\rangle\Big)/2.
    \end{split}
\end{equation}
Similarly we can apply a controlled $\hat{X}^{1, 2}\hat{Z}^2\hat{X}^{0, 1}$ and get the state
\begin{equation}
    \label{eq:timeevolvedxzx}
    \begin{split}
        |\Psi''_{xzx}(y)\rangle &= \Big(
    |1\rangle \hat{X}^{1, 2}_y \hat{X}^{0, 1}_y\hat{Z}^2_y e^{-it\hat{H}}\hat{U}^+_x|\psi_i\rangle\\
    &+|0\rangle e^{-it\hat{H}}|\psi_j\rangle\Big)/2.
    \end{split}
\end{equation}
Finally, measuring the ancilla for the states given in Eqs. (\ref{eq:timeevolvedxx}) and (\ref{eq:timeevolvedxzx}) in the $\hat{\sigma}^x$ or $\hat{sigma}^y$ basis will yield the real or imaginary parts respectively of the quantities,
\begin{equation}
\label{eq:timeevolvedhermitianterms}
    \begin{split}
        T_{xx}(y) &= \langle \psi_j | e^{i t \hat{H}} \hat{X}^{1, 2}_y \hat{X}^{0, 1}_y e^{-it\hat{H}}\hat{U}^+_x|\psi_i\rangle \\ 
        T_{xzx}(y) &= \langle \psi_j | e^{i t \hat{H}} \hat{X}^{1, 2}_y \hat{Z}_y^2\hat{X}^{0, 1}_y e^{-it\hat{H}}\hat{U}^+_x|\psi_i\rangle. 
    \end{split}
\end{equation}
It clearly follows that the sum of these two terms gives us the desired correlator. These operations can be expressed as the following quantum circuits: 
\begin{widetext}
\begin{equation}
    \label{eq:stateprep}
    \begin{split}
    \begin{gathered}
    \Qcircuit @C=1.5em @R=1em {
    \lstick{|+\rangle} & \ctrlo{1} & \ctrl{1} & \qw & \ctrl{1} & \ctrl{1} & \qw & \measure{\mbox{$\sigma^x$ \text{ or } $\sigma^y$}}\\
    \lstick{|0...0\rangle} & \gate{\hat{V}_j} & \gate{\hat{W}_i} & \gate{e^{-i t \hat{H}}} & \gate{X^{0, 1}_y} & \gate{X^{1, 2}_y} & \qw & \qw \\ 
    }
    \end{gathered} & = T_{xx}(y) \text{ and }\\
    \begin{gathered}
    \Qcircuit @C=1.5em @R=1em {
    \lstick{|+\rangle} & \ctrlo{1} & \ctrl{1} & \qw & \ctrl{1} & \ctrl{1} & \ctrl{1} & \qw & \measure{\mbox{$\sigma^x$ \text{ or } $\sigma^y$}}\\
    \lstick{|0...0\rangle} & \gate{\hat{V}_j} & \gate{\hat{W}_i} & \gate{e^{-i t \hat{H}}} & \gate{Z^2} & \gate{X^{0, 1}_y} & \gate{X^{1, 2}_y} & \qw & \qw \\ 
    }
    \end{gathered} & = T_{xzx}(y).
    \end{split}
\end{equation}
\end{widetext}
It will be shown in the rest of this section the demonstration of an emulation of a NISQ era qutrit based quantum computer. 

We can extract information regarding the propogator from a real time simulation in the following manner:
\begin{equation}
    G(E, \vec{p}) = \int_{0}^{\infty}dt \sum_{\vec{x}} \langle C(\vec{x}, t) e^{-i E t + i \vec{p} \cdot \vec{x}}.
\end{equation}
In practice the integral over $t$ can be truncated to some $t_max$. 

==> qubit_encoding.tex <==


